The static parallel distribution algorithms for hybrid density-functional calculations in HONPAS package

Hybrid density-functional calculation is one of the most commonly adopted electronic structure theory used in computational chemistry and materials science because of its balance between accuracy and computational cost. Recently, we have developed a novel scheme called NAO2GTO to achieve linear scaling (Order-N) calculations for hybrid density-functionals. In our scheme, the most time-consuming step is the calculation of the electron repulsion integrals (ERIs) part. So how to create an even distribution of these ERIs in parallel implementation is an issue of particular importance. Here, we present two static scalable distributed algorithms for the ERIs computation. Firstly, the ERIs are distributed over ERIs shell pairs. Secondly, the ERIs is distributed over ERIs shell quartets. In both algorithms, the calculation of ERIs is independent of each other, so the communication time is minimized. We show our speedup results to demonstrate the performance of these static parallel distributed algorithms in the Hefei Order-N packages for \textit{ab initio} simulations (HONPAS).

==> Makefile <==
base_name := manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))

%.dvi: %.tex
	latex --interaction=nonstopmode $<
	latex --interaction=nonstopmode $<
#	makeindex -s index-style.ist $*.idx
	bibtex $*.aux
	latex --interaction=nonstopmode $<
	latex --interaction=nonstopmode $<

%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<
#	makeindex -s index-style.ist $*.idx
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<

%.ps: %.dvi
	dvips $<

all: $(base_name).pdf  
	(evince $(base_name).pdf  &)
pdf: $(base_name).pdf
ps:  $(base_name).ps
display: 
	evince $(base_name).pdf 


$(base_name).pdf: $(base_name).tex mybib.bib 


dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

clean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib


.PHONY: clean  backup

